Transfer Learning of Graph Neural Networks with Ego-graph Information Maximization

Graph neural networks (GNNs) have achieved superior performance in various applications, but training dedicated GNNs can be costly for large-scale graphs. Some recent work started to study the pre-training of GNNs. However, none of them provide theoretical insights into the design of their frameworks, or clear requirements and guarantees towards their transferability. In this work, we establish a theoretically grounded and practically useful framework for the transfer learning of GNNs. Firstly, we propose a novel view towards the essential graph information and advocate the capturing of it as the goal of transferable GNN training, which motivates the design of EGI (Ego-Graph Information maximization) to analytically achieve this goal. Secondly, when node features are structure-relevant, we conduct an analysis of EGI transferability regarding the difference between the local graph Laplacians of the source and target graphs. We conduct controlled synthetic experiments to directly justify our theoretical conclusions. Comprehensive experiments on two real-world network datasets show consistent results in the analyzed setting of direct-transfering, while those on large-scale knowledge graphs show promising results in the more practical setting of transfering with fine-tuning.

==> archiv.tex <==
\begin{table*}[h]
\begin{center}
    

\caption{Results of role identification with direct-transfering on the Airport dataset. The performance is the average over 100 runs. The scores marked with $^{**}$ passed t-test with $p < 0.01$ over the second best results.}
\label{tab:role-classification}
\scalebox{0.9}{
\begin{tabular}{lll|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\multirow{2}{*}{Method}}                             & \multicolumn{2}{c|}{Europe (source)} & \multicolumn{2}{c|}{USA (target)} & \multicolumn{2}{c}{Brazil (target)}                                                                                                            \\
\multicolumn{3}{c|}{}                                                    & node degree & uniform & node degree & uniform & node degree & uniform \\ \midrule

\multicolumn{2}{l}{}                              & features &  52.81         &   20.59       &   55.67      &  20.22 & 67.11 & 19.63 \\

%\multicolumn{2}{l}{}                              & GCN (untrained)                    &  52.96       &  20.11       &  55.30       &  22.07 & 68.30 & 17.63  \\

\multicolumn{2}{l}{}                              & GIN (untrained)                    &  55.75   &   53.88       &    61.56      &  58.32  & 70.04 & 70.37\\
\multicolumn{2}{l}{}                              & GVAE~\cite{kipf2016variational}                  &  53.90    &   21.12      &  55.51       &  22.39 & 66.33 & 17.70                            \\
\multicolumn{2}{l}{}                              & DGI~\cite{velivckovic2018deep}                   &  57.75      &    22.13     &  54.90      &  21.76 & 67.93 & 18.78                          \\
\multicolumn{2}{l}{}                              & MaskGNN~\cite{hu2019strategies}                   &  56.37      &  55.53        &      60.82 & 54.64 & 66.71 &74.54                     \\
\multicolumn{2}{l}{}                              & ContextPredGNN~\cite{hu2019strategies}                    &  52.69       &   49.95       &  50.38      & 54.75  & 62.11 & 70.66                       \\
\multicolumn{2}{l}{}                              & Structural Pre-train~\cite{hu2019pre}                   & 56.00       &   53.83      &    62.17    & 57.49  & 68.78 &  72.41                     \\
\multicolumn{2}{l}{}                              & MVC~\cite{hassani2020contrastive}                    &    53.16    &   51.69     &  59.66  & 50.42   &  66.07   & 61.55                    \\
\multicolumn{2}{l}{}                              & GMI~\cite{peng2020graph}                   & 58.12       &   46.25      &   59.28     & 47.64  & 73.07   &  62.96                     \\
\multicolumn{2}{l}{}                              & \Ours                   & \textbf{59.15}$^{**}$       &  54.98 &\textbf{64.55}$^{**}$      &   57.40    &  \textbf{73.15} & 70.00                       \\
\bottomrule

\end{tabular}
}
\end{center}
\end{table*}

==> prelim.tex <==
\section{Problem Definition \& Preliminary }

\QZ{Removed the below content in the previous draft and merge them mostly to the method part. Featureless claims make ppl uncomfortable.} 

\DEL{
In the most general graph transfer learning setting, where both downstream tasks and node features can be unknown and changeable between pre-training and transfering, it remains an important problem to optimize and quantify the utility of GNNs across different graphs in an \textit{unsupervised} and \textit{featureless} setting.
}

\DEL{
Formally, transfer learning of GNN considers a graph $G=\{V, E\}$, where the set of nodes $V$ are associated with certain features and the set of links $E$ form certain structures. Under an \textit{unsupervised-transfering setting}, we consider a GNN $\Psi$ to be pre-trained on a source graph $G_a$ and applied on a target graph $G_b$ \textit{without fine-tuning}.
The transferability of a GNN can then be evaluated based on the difference between the unsupervised losses on the source and target graphs. 
Unlike existing studies on GNN pre-training, which only consider a particular downstream task and requires it to be the same on source and target graphs \cite{hu2019strategies, hu2019pre}, our study is more general towards the core function of GNNs in graph structure learning.
}

\DEL{
In real life, the majority of graph data, especially where GNN pre-training has been considered as valuable, are featureless, such as brain networks, gene networks, as well as the REDDIT and IMDB social networks~\cite{yanardag2015deep}. Same as most existing studies on graph theory, in this work, we start with graphs without the possibly complex and noisy organic node features like user/item profiles, but derive the more analyzable structure relevant features like node degrees as the input of GNNs.
}

\DEL{
Note that, although we focus our theoretical studies on the unsupervised and featureless setting, our empirical analysis shows our model and its guarantee to be naturally extensible to the more practical settings of transfering with task-specific fine-tuning and node features, especially when the tasks and features are structure relevant. 
}

==> supps/macro.tex <==
\usepackage{amsmath, amsfonts, amssymb, xspace, color, amsbsy, caption, adjustbox, amsthm}
\usepackage{tabularx}
% \usepackage{tikz, graphicx, algorithmic, capt-of, ifthen, calc, algorithm}
\usepackage{tikz, graphicx}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{cleveref}
%\usepackage{subfig}
\usetikzlibrary{positioning}
\usepackage[linesnumbered,ruled,lined]{algorithm2e}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{subcaption}
%,labelfont=bf,textfont=bf
\usepackage{esvect}

\usepackage{changepage}
\usepackage{pifont}
%\theoremstyle{definition}
\theoremstyle{plain}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{thm:eg}{Example}
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}

\newcommand{\Ours}{\textsc{Egi}\xspace}
\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1}}}
\newcommand{\tick}{\ding{52}}
% ----------------------------------------------------------------------
% For draft editing.
% ----------------------------------------------------------------------

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
% \newcommand{\hide}[1]{} %hide
\newcommand{\vpara}[1]{\vspace{0.01in}\noindent\textbf{#1}}
\newcommand{\para}[1]{\vspace{0.1in}\noindent\textbf{#1}}
\newcommand{\pa}[2]{\vspace{#1}\noindent\textbf{#2}} % a new paragraph without indent
\newcommand{\benum}[1]{\begin{enumerate}#1\end{enumerate}}
\newcommand{\bitem}[1]{\begin{itemize}#1\end{itemize}}

\newcommand{\ulpara}[1]{\vspace{0.01in}\noindent\emph{#1}}

% ----------------------------------------------------------------------
%  Common abbreviations and words with accents
% ----------------------------------------------------------------------

\newcommand{\etal}{\emph{et~al.}\xspace} % and others
\newcommand{\ie}{\emph{i.e.}\xspace} % that is
\newcommand{\eg}{\emph{e.g.}\xspace} % for example
\newcommand{\etc}{\emph{etc.}\xspace} % that is
\newcommand{\wrt}{\emph{w.r.t.}\xspace} % with respect to
\newcommand{\iid}{\emph{i.i.d.}\xspace}

\newcommand{\naive}{na\"{\i}ve\xspace} % and others
\newcommand{\Naive}{Na\"{\i}ve\xspace} % and others
\newcommand{\ssym}{§}

% ----------------------------------------------------------------------
% Math symbols.
% ----------------------------------------------------------------------

\newcommand{\beal}[1]{\begin{align}#1\end{align}}
\newcommand{\beq}[1]{\begin{equation}#1\end{equation}}
\newcommand{\beqn}[1]{\begin{eqnarray}#1\end{eqnarray}}

\newcommand{\Sum}{\sum\limits} % Cheap displaystyle operators
\newcommand{\Max}{\max\limits}
\newcommand{\Min}{\min\limits}
\newcommand{\Prod}{\prod\limits}
\newcommand{\Lim}{\lim\limits}
\newcommand{\Bcup}{\bigcup\limits}

\newcommand{\abs}[1]{\mathopen| #1 \mathclose|}			% use instead of $|x|$
\newcommand{\norm}[1]{\mathopen\| #1 \mathclose\|}			% use instead of $\|x\|$
\newcommand{\inner}[2]{\langle #1, #2 \rangle}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\def \E {\mathrm{E}}

\def \c {\mathbf{c}}
\def \d {\mathbf{d}}
\def \e {\mathbf{e}}
\def \f {\mathbf{f}}
\def \g {\mathbf{g}}
\def \h {\mathbf{h}}
\def \l {\mathbf{l}}
\def \m {\mathbf{m}}
\def \o {\mathbf{o}}
\def \p {\mathbf{p}}
\def \q {\mathbf{q}}
\def \r {\mathbf{r}}
\def \t {\mathbf{t}}
\def \u {\mathbf{u}}
\def \v {\mathbf{v}}
\def \w {\mathbf{w}}
\def \x {\mathbf{x}}
\def \y {\mathbf{y}}
\def \z {\mathbf{z}}
\def \A {\mathbf{A}}
\def \H {\mathbf{H}}
\def \I {\mathbf{I}}
\def \L {\mathbf{L}}
\def \P {\mathbf{P}}
\def \U {\mathbf{U}}
\def \W {\mathbf{W}}

\def \B {\mathcal{B}}
\def \C {\mathcal{C}}
\def \D {\mathcal{D}}
\def \F {\mathcal{F}}
\def \M {\mathcal{M}}
\def \N {\mathcal{N}}
\def \O {\mathcal{O}}
\def \Q {\mathcal{Q}}
\def \R {\mathcal{R}}
\def \S {\mathcal{S}}
\def \T {\mathcal{T}}
\def \calX {\mathcal{X}}
\def \calY {\mathcal{Y}}
\def \calH {\mathcal{H}}
\def \calL {\mathcal{L}}

\def \X {\mathbf{X}}
\def \Y {\mathbf{Y}}
\def \Z {\mathbf{Z}}

\def \RR {\mathbb{R}}
\def \NN {\mathbb{N}}
\def \SSS {\mathbb{S}}
\def \regret {\mbox{regret}}
\def \Uh {\widehat{U}}

\def \sig {\sigma}
\def \gt {g_{\theta}}
\def \gi  {g_i}
\def \gid {g_{i'}}
\def \fj  {f_{j}}
\def \fjd {f_{j'}}

% ----------------------------------------------------------------------
% Document-specific commands.
% ----------------------------------------------------------------------
\newcommand{\ADD}[1]{\textcolor{red}{Added: #1}}
\newcommand{\DEL}[1]{\textcolor{blue}{Deleted: #1}}
\newcommand{\QZ}[1]{\textcolor{orange}{Bran: #1}}
\newcommand{\carl}[1]{\textcolor{purple}{Carl: #1}}


\def \zero {\mathbf{0}}
\def \one {\mathbf{1}}
\def \PT {\mathbf{P}^\text{T}}

\newcommand{\hop}{\texttt{Hop}\xspace}
\newcommand{\SP}{\texttt{SP}\xspace}
\newcommand{\RWR}{\texttt{RWR}\xspace}
\newcommand{\wave}{\textsc{Wavelet}\xspace}
\newcommand{\our}{\textsc{AFGRE}\xspace}
\newcommand{\iknn}{\textsc{Ink}\xspace}
\newcommand{\knn}{top-$k$\xspace}
\newcommand{\rd}[1]{^{(#1)}}
\newcommand{\lb}[1]{\underline{#1}\xspace}
\newcommand{\ub}[1]{\overline{#1}\xspace}


% Shrink space.
% \setlength{\floatsep}{4pt plus 4pt minus 1pt}
% \setlength{\textfloatsep}{4pt plus 2pt minus 2pt}
% \setlength{\intextsep}{4pt plus 2pt minus 2pt}

% \setlength{\dbltextfloatsep}{3pt plus 2pt minus 1pt}
% \setlength{\dblfloatsep}{3pt plus 0pt minus 0pt}

% \setlength{\abovedisplayskip}{2pt plus 1pt minus 1pt}
% \setlength{\belowdisplayskip}{2pt plus 1pt minus 1pt}


% ----------------------------------------------------------------------
% Commands used in clustering.
% ----------------------------------------------------------------------


\def \Kappa {\boldsymbol{\kappa}}
\def \sS {\mathbf{S}}
\def \sX {\mathcal{X}}
\def \sz {\mathcal{Z}}
\def \Mu {\boldsymbol{\mu}}
\def \Eta {\boldsymbol{\eta}}
\def \vmf {\mathbf{vMF}}
\def \cluster {\textsc{Shifting-Window Clustering }}

\SetKwRepeat{Do}{do}{while}
